Unlocking Out-of-Distribution Generalization in Transformers via Recursive Latent Space Reasoning

Systematic, compositional generalization beyond the training distribution remains a core challenge in machine learning -- and a critical bottleneck for the emergent reasoning abilities of modern language models. This work investigates out-of-distribution (OOD) generalization in Transformer networks using a GSM8K-style modular arithmetic on computational graphs task as a testbed. We introduce and explore a set of four architectural mechanisms aimed at enhancing OOD generalization: (i) input-adaptive recurrence; (ii) algorithmic supervision; (iii) anchored latent representations via a discrete bottleneck; and (iv) an explicit error-correction mechanism. Collectively, these mechanisms yield an architectural approach for native and scalable latent space reasoning in Transformer networks with robust algorithmic generalization capabilities. We complement these empirical results with a detailed mechanistic interpretability analysis that reveals how these mechanisms give rise to robust OOD generalization abilities.

==> figs/architecture_diagram_unrolled.tex <==
\begin{tikzpicture}[>=Latex, line width=0.8pt,
    every node/.style={font=\small}]

% bright
% ['#4477AA', '#EE6677', '#228833', '#CCBB44', '#66CCEE', '#AA3377', '#BBBBBB']%
% vibrant
% ['#EE7733', '#0077BB', '#33BBEE', '#EE3377', '#CC3311', '#009988', '#BBBBBB']%
% light
% ['#77AADD', '#EE8866', '#EEDD88', '#FFAABB', '#99DDFF', '#44BB99', '#BBCC33', '#AAAA00', '#DDDDDD']

%––– colours selected from the “vibrant” palette
\definecolor{transformerblockcol}{HTML}{0077BB}
\definecolor{bottleneckcolor}{HTML}{009988}
\definecolor{supervisioncolor}{HTML}{EE3377}

% Enable grid
% \draw[step=0.5cm,gray!30,very thin] (-2,-3) grid (14,3);

%% Input arrow & label
\draw[->] (-1,0) -- (0,0);
\node[left=2pt] at (-1,0) {\textit{Input}};

%% Block 1 – Transformer (no internal text)
\draw[fill=transformerblockcol, draw=none] (0,1.5) rectangle (1,-1.5);

%% Arrow to Bottleneck 1
\draw[->] (1,0) -- (2,0);

%% Bottleneck 1 – Discretize / Re-Embed trapezoids (no internal text)
\draw[fill=bottleneckcolor, draw=none] % draw=none omits border outline
(2,1.5) -- (2,-1.5) -- (2.9,-0.75) -- (2.9,0.75) -- cycle;
\draw[fill=bottleneckcolor, draw=none]
(4,1.5) -- (4,-1.5) -- (3.1,-0.75) -- (3.1,0.75) -- cycle;


%% ---- hatched rectangle between the two trapezoids ----
\path[
      pattern=north east lines,   % hatch direction
      pattern color=supervisioncolor,          % hatch strokes in red
      draw = none,
    %   draw opacity=0,
      fill opacity=100
     ]
     (2.9, 0.75) rectangle (3.1, -0.75);

%% Label underneath hatching
\node[below=2pt, text=supervisioncolor] at (3,-1.5) {\footnotesize{\textit{Latent Space Supervision}}};

%% Arrow to Block 2
\draw[->] (4,0) -- (5,0);

%% Block 2 – Transformer
\draw[fill=transformerblockcol, draw=none] (5,1.5) rectangle (6,-1.5);

%% Ellipsis & continuation arrow
\draw[->] (6,0) -- (7.25,0);
\node at (7.7,0) {$\cdots$};
\draw[->] (8.15,0) -- (9.15,0);

%% Block 3 – Transformer
\draw[fill=transformerblockcol, draw=none] (9.15,1.5) rectangle (10.15,-1.5);

%% Arrow to Bottleneck 2
\draw[->] (10.15,0) -- (11.15,0);

%% Bottleneck 2 – unlabeled trapezoids
\draw[fill=bottleneckcolor, draw=none]
(11.15,1.5) -- (11.15,-1.5) -- (12.05,-0.75) -- (12.05,0.75) -- cycle;
\draw[fill=bottleneckcolor, draw=none]
(13.15,1.5) -- (13.15,-1.5) -- (12.25,-0.75) -- (12.25,0.75) -- cycle;

%% Auxiliary arrows & text
\draw[dashed] (3,1.675) -- (3,-1.575);
\node[above] at (3,1.75) {\textit{Discrete Bottleneck}};
% \node[above] at (3,3) {Latent Reasoning\\Supervision};

% \draw[->] (3,-0.3) -- (3,-2.3);
% \node[below=2pt] at (3,-2.3) {Discretise into Binned\\Latent Code};

%% ------------------------------------------------------------------
%% Legend  -----------------------------------------------------------
%% ------------------------------------------------------------------
\begin{scope}[yshift=-2.75cm, xshift=1.5cm]
% Transformer block legend entry
\draw[fill=transformerblockcol, draw=none] (0,0.25) rectangle (0.3,-0.25);
\node[right=3pt] at (0.3,0) {\footnotesize{\textit{Recurrent Transformer Block}}};

% Discretize trapezoid legend entry
\draw[fill=bottleneckcolor, draw=none]
(4.5,0.25) -- (4.5,-0.25) -- (4.8,-0.125) -- (4.8,0.125) -- cycle;
\node[right=3pt] at (4.8,0) {\footnotesize{\textit{Discretize}}};

% Re-Embed trapezoid legend entry (mirrored)
\draw[fill=bottleneckcolor, draw=none]
(6.6,0.125) -- (6.6,-0.125) -- (6.9,-0.25) -- (6.9,0.25) -- cycle;
\node[right=3pt] at (6.9,0) {\footnotesize{\textit{Re-Embed}}};
\end{scope}

\end{tikzpicture}


==> figs/dag_example.tex <==
\begin{tikzpicture}[
    node distance=0.7cm and 2.0cm, % Vertical and horizontal distance
    var/.style={draw, circle, minimum size=0.7cm, inner sep=1pt, thick}, % Variable nodes
    val/.style={font=\scriptsize}, % Input value nodes
    arr/.style={->, >=Stealth[], thick} % Arrows
]
    % Input values are still random for leaf nodes
    % \pgfmathsetseed{101} % Optional: for reproducible random input values

    % ----- Layer 1: Leaf Nodes -----
    \node[var] (l1n1) {$x_{7}$}; % Hard-coded index
    \node[val, left=0.4cm of l1n1] (v1) {20};
    \draw [arr] (v1) -- (l1n1);

    \node[var, below=of l1n1] (l1n2) {$x_{42}$}; % Hard-coded index
    \pgfmathrandominteger{\rv}{0}{23}
    \node[val, left=0.4cm of l1n2] (v2) {2};
    \draw [arr] (v2) -- (l1n2);

    \node[var, below=of l1n2] (l1n3) {$x_{88}$}; % Hard-coded index
    \pgfmathrandominteger{\rv}{0}{23}
    \node[val, left=0.4cm of l1n3] (v3) {6};
    \draw [arr] (v3) -- (l1n3);

    \node[var, below=of l1n3] (l1n4) {$x_{115}$}; % Hard-coded index
    \pgfmathrandominteger{\rv}{0}{23}
    \node[val, left=0.4cm of l1n4] (v4) {14};
    \draw [arr] (v4) -- (l1n4);

    % ----- Layer 2: Intermediate Nodes -----
    \node[var, right=of $(l1n1)!0.5!(l1n2)$] (l2n1) {$x_{23}$}; % Hard-coded index

    \node[var, right=of $(l1n2)!0.5!(l1n3)$] (l2n2) {$x_{91}$}; % Hard-coded index

    \node[var, right=of $(l1n3)!0.5!(l1n4)$] (l2n3) {$x_{55}$}; % Hard-coded index


    % ----- Layer 3: Output Nodes -----
    \node[var, right=of $(l2n1)!0.5!(l2n2)$] (l3n1) {$x_{101}$}; % Hard-coded index

    \node[var, right=of $(l2n2)!0.5!(l2n3)$] (l3n2) {$x_{30}$}; % Hard-coded index


    % ----- Edges Layer 1 -> Layer 2 -----
    \draw [arr] (l1n1) -- (l2n1); % x7 -> x23
    \draw [arr] (l1n2) -- (l2n1); % x42 -> x23
    \draw [arr] (l1n2) -- (l2n2); % x42 -> x91
    \draw [arr] (l1n3) -- (l2n2); % x88 -> x91
    \draw [arr] (l1n3) -- (l2n3); % x88 -> x55
    \draw [arr] (l1n4) -- (l2n3); % x115 -> x55
    \draw [arr] (l1n1) -- (l2n2); % x7 -> x91

    % ----- Edges Layer 2 -> Layer 3 -----
    \draw [arr] (l2n1) -- (l3n1); % x23 -> x101
    \draw [arr] (l2n2) -- (l3n1); % x91 -> x101
    \draw [arr] (l2n2) -- (l3n2); % x91 -> x30
    \draw [arr] (l1n3) -- (l3n2); % x55 -> x30
    \draw [arr] (l2n3) -- (l3n2); % x55 -> x30
    % \draw [arr] (l2n1) -- (l3n2); % x23 -> x30

    % ----- Description Node -----
    \node (desc) [below=1.5cm of $(l1n4)!0.5!(l3n2)$, text width=15cm, align=center, font=\small] {

        $\token{20} \token{\to} \token{x_7} \sep \token{2} \token{\to} \token{x_{42}} \sep \token{6} \token{\to} \token{x_{88}} \sep \token{14} \token{\to} \token{x_{115}} \sep$

        $\token{x_7} \oper \token{x_{42}} \token{\to} \token{x_{23}} \sep \token{x_7} \oper \token{x_{42}} \oper \token{x_{88}} \token{\to} \token{x_{91}} \sep \token{x_{88}} \oper \token{x_{115}} \token{\to} \token{x_{55}} \sep$

        $\token{x_{23}} \oper \token{x_{91}} \token{\to} \token{x_{101}} \sep \token{x_{91}} \oper \token{x_{88}} \oper \token{x_{55}} \token{\to} \token{x_{30}}$
    };

\end{tikzpicture}


==> methods_old.tex <==
\section{Methods \& Experiments}

\subsection{Task: Mathematical Reasoning on Computation Graphs}

\aanote{This is a rough first draft. TODO -- revise and write polished version for paper.}

In this work, we focus our study on a task based on mathematical reasoning on computation graphs, allowing us to study the out-of-distribution generalization capabilities of Transformer networks by training on small-sized computational graphs and testing on larger graphs.

\textbf{Task Description.} A computation graph is a representation of a network of mathematical computation as a directed acyclic graph, where the nodes correspond to variables and the edges describe the flow of information and the dependency between variables. The inputs to each node, represented as in-flowing edges, are the variable values needed to compute the node. The out-flowing edges from a node represent the subsequent nodes that require that variable's value to perform their calculation. Each node can be computed using the values of the nodes it depends on and a specification of the operations or functions relating them. In our experiments, the operations are modular arithmetic (addition, multiplication, subtraction) modulo $23$.

\textbf{Data Generation Process.} The following task parameters are specified: graph size (i.e., \# of nodes $N$), number of leaf nodes $L$, set of operations (e.g., $\calO = \sset{+, -, \times}$), set of variable names (e.g., $\calV = \sset{x_{1}, \ldots, x_{128}}$), and a set of numerical values (e.g., $\calN = \sset{0, 1, \ldots, 23}$). Input instances are randomly generated as follows.
\begin{enumerate}
    \item Randomly generate a directed acyclic graph with $N$ nodes, $L$ of which are leaf nodes.
    \item Randomly assign a variable name to each node.
    \item Randomly assign numerical values to the leaf nodes.
\end{enumerate}

The input instances are presented to the model as a sequence of tokens. Each variable name, numerical value, and operation is assigned a unique token. This is depicted in~\Cref{fig:dag_example}.

\textbf{Target output \& Evaluation Metric.} The task is to compute the value of every node in the computation graph. Throughout the paper, we focus on the most stringent possible evaluation metric: the full sequence accuracy (i.e., the proportion of inputs where the value of \textit{all} nodes in the graph is computed correctly).


\aanote{Maybe add a figure that shows a representation of the contrast between the training and testing distribution in terms of graph size. E.g., on the left a graph with $32$ nodes and on the right a graph with $128$ nodes to visually represent the increase in size.}



\zynote{This figure is too ugly. We need to make it look nicer. Use different colors for different types of nodes. Do not use Latex. Use other drawing tools. Also, use a better format for the token sequences. Use colors. Also, write the mathematical equations, and the tokens. Put them in a box and put that box to the right of the graph.}

\begin{figure}
    \centering
    \input{figs/dag_example.tex}
    \caption{\textbf{Top.} A depiction of an instance in our mathematical reasoning task. A directed acyclic graph is randomly generated, each node is assigned a variable name label, and leaf nodes are randomly assigned values. Operations are also randomly sampled, which in our setting our arithmetic operations such as addition, multiplication, etc. \textbf{Bottom.} The token representation of the computation graph.}
    \label{fig:dag_example}
\end{figure}





\textbf{Out-of-Distribution Generalization.} Our main focus in this work is on probing the ability of Transformer networks to learn general problem-solving procedures and algorithms that allow them to generalize \textit{out-of-distribution}. In our mathematical reasoning task, this is formulated by training on problem instances with $N \leq 32$ nodes, and test on problem instances of varying size, up to four times larger at $N = 128$. This is a particularly challenging form of OOD generalization because it requires generalization not only in length, but also in computational depth.


\begin{itemize}
    \item \textbf{\textit{Length Generalization}.} The problem instances in the OOD splits involve larger graphs, and therefore longer inputs. The model must be able to handle inputs oof varying lengths in its attention mechanism, and avoid misleading heuristics tied to the length of the training data.
    \item \textbf{\textit{Depth Generalization}.} The problem instances in the OOD split are not only longer, but they also require a larger number of parallel computational steps to compute. That is, the graphs themselves are deeper, and hence require the model to traverse greater depths to compute nodes in deeper layers.
\end{itemize}


{\color{red} It seems hard to understand the difference between length and depth generalization. I think we should clarify this. }
\aanote{e.g., mention communication theoretic analysis for lower bounds, etc. e.g., recent work has used this to show that induction heads require depth $\geq 2$.}

% Properties of task:
% \begin{itemize}
%     \item Representative of mathematical reasoning
%     \item Allows us to study different types of generalization (out-of-distribution, length generalization, depth generalization, easy-to-hard generalization). Synthetic and therefore very tunable.
%     \item 
% \end{itemize}

\subsection{Motivation: Transformers Fail to Generalize Out-of-Distribution}


{\color{red} Give a few names to the methods we are going to compare against. Vanilla trasformers, CoT, etc.}


\aanote{Should we also mention that (weaker) baseline of end-to-end models also fail? Those are weaker baselines and perhaps not too surprising. I wonder what the best way to present this section is?}


\zynote{Do not need to capitalize "Transforemrs". Use "transformers". }


To motivate our findings, let us first attempt to solve this task via standard architectures and training techniques. A common approach to train Transformer-based language models to perform multi-step reasoning is autoregressive chain-of-thought training. Rather than directly outputting the final answer, this approach involves training a model to autoregressively generate the solution step-by-step in a sequential manner. This enables providing the model with rich and detailed supervision for each individual computational step, and has been shown to yield significantly improved performance on multi-step reasoning tasks, including mathematical reasoning~\cite{...}.

We begin by training causal Transformer language models on chain-of-thought trajectories that represent computing the nodes in the given computation graph one by one. The input prompt to the model is a token representation of the computation graph, as depicted in~\Cref{fig:dag_example}. This is followed by a special $\token{\mathtt{CoT}}$ token that denotes the beginning of the chain-of-thought, followed by step-by-step computation of the nodes in the graph. The chain-of-thought trajectory computes each node in the graph, in topological order, first recalling the equation defining the value of the node, then recalling the values of the dependent nodes, and finally performing the arithmetic computation. For example, to compute node $\token{x_{101}}$ in \Cref{fig:dag_example}, the chain-of-thought trajectory has the following form.
\begin{equation*}
    \mathtt{[...Input\, Prompt...]} \token{\mathtt{CoT}} [...] \token{x_{101}} = \token{x_{23}} \ADD \token{x_{91}} = \token{22} \ADD \token{5} = \token{4}
\end{equation*}
Here, the preceding portion of the chain-of-thought trajectory $[...]$ already computed the values of $\token{x_{23}}$ and $\token{x_{91}}$. Recall that $\ADD$ denotes modular addition, mod $23$, and each numerical value between $0$ and $22$ is encoded as a unique token.

We train a causal Transformer language model on chain-of-thought trajectories solving randomly generated problem instances from our task with graph size $N \leq 32$. At inference time, we prompt the model with only the input, and autoregressively generate the solution (using greedy decoding). We evaluate the model on new randomly generated inputs corresponding to graphs of varying size, and compute the proportion of inputs where the model correctly computes all nodes in the graph. We compare this to end-to-end models, both feedforward and recurrent, that are trained to directly output the entire solution in a single forward pass. For each method, we perform an in-depth hyperparameter search over the number of layers, model dimension, and positional encoding method, selecting the best model for comparison against different methods.

We find that chain-of-thought training enables the model to learn to solve larger graphs, compared to end-to-end models without chain-of-thought supervision, but can only generalize \textit{in-distribution}. The models are able to generalize out-of-distribution to larger graphs to a limited degree, but this ability quickly degrades as the graphs increase in size beyond the training distribution. Although hyperparameter choice---namely model depth and the choice of positional encoding method--- has a significant effect on model performance, the failure to generalize to the OOD split persists across of hyperparameter choice. We provide a detailed description of the experimental setup for these experiments in~\Cref{sec:cot_details}.

% \begin{figure}
%     \centering
%     % \includegraphics[width=\linewidth]{figs/experiment_results/method_ood_comparison/method_ood_comparison_legendtop.pdf}
%     \includegraphics[width=\linewidth]{figs/experiment_results/method_ood_comparison/method_ood_comparison.pdf}
%     \caption{Out-of-Distribution generalization performance of different methods on the mathematical reasoning task.}
%     \label{fig:method_ood_comparison}
% \end{figure}

\subsection{Architectural Ingredients for Robust OOD Generalization.}

\begin{figure}
    \centering
    \resizebox{\linewidth}{!}{
    \input{figs/architecture_diagram.tex}
    }
    % \input{figs/architecture_diagram.tex}
    \caption{[[Depiction of Architecture.]]}
\end{figure}

In this section, we reflect on the failure of standard methods, such as CoT supervision, to robustly generalize out-of-distribution on this task, and propose a series of architectural and algorithmic \aanote*{mechanisms?}{methods} that enable robust generalization in length and depth on this task. We show that the resulting method achieves near-perfect robust out-of-distribution generalization. We then discuss the implications of our findings to out-of-distribution generalization in neural networks more broadly, and to settings of real-world interest in the context of Transformer-based language models.


{\color{red}  Write a paragraph that points out why the previous methods fail. Use a short subtitle. } 


{\color{red}  Then motivate our method. When introducing our methods, write in paragraphs with short subtitles. (This is our current style.) But try to add equations or examples. Currently the text is full of text and hard to understand for people who only spend 10 min reading.} 


% We propose four key ingredients to enable robust OOD generalization: (1) algorithmic supervision of latent representations, (2) recurrence and input-adaptive scaling of computation, (3) latent representation pinning via discretization, and (4) self-correction mechanisms.

\aanote{This paragraph needs to be refined and better-motivated. Maybe need some discussion before. The proposal needs to be made more clear.}

\textbf{\textit{Algorithmic Supervision of Latent Representation}.}
A key factor that determines whether a neural network is able to generalize is how well it is aligned to a robust \textit{algorithm} for solving the task. In particular, to solve the task on a specific distribution, gradient-based training may find a collection of heuristics and shortcuts that achieve good or perfect performance on the training distribution, but, once we deviate from the training distribution (e.g., to larger problem instances), these heuristics \aanote*{collapse?}{no longer apply} and model performance rapidly degrades. To achieve robust generalization, it is necessary to imbue the architecture and/or optimization procedure with a set of \textit{inductive biases} that steer the learning process towards solutions that represent robust and scalable problem-solving algorithms. Chain-of-thought supervision is the standard means of achieving this in Transformer networks, whereby an autoregressive model is trained to sequentially predict each step of some underlying reasoning process. However, as we see in~\Cref{fig:method_ood_comparison}, while this enables good in-distribution performance, improving significantly over the end-to-end baselines, these methods do not robustly generalize outside the training distribution. This can partly be attributed to length generalization, which is a central challenge and limitation of Transformer networks that has been studied extensively in prior work~\cite{kazemnejadImpactPositionalEncoding2023,zhouWhatAlgorithmsCan2023,jelassi2023lengthgeneralizationarithmetictransformers,zhouTransformersCanAchieve2024}. Moreover, we argue that standard Chain-of-Thought techniques suffer from the fundamental limitation that it restricts the reasoning path to a single linear \textit{chain}, which may not align with the intrinsic structure of the task. 
% which can be inefficient and misaligned for many important tasks (including the mathematical reasoning task we consider in this work), missing out on the parallelism of Transformer networks, which is one of the architecture's inherent strengths.
{\color{red} The above paragraph is all about the challenge of previous methods, but not what we propose.}
% Implementation: we train prediction heads to predict the outputs of the values that are computable at that depth, and add the loss of these heads to the overall loss. This trains the model to reason one layer at a time on the input graph, computing values one layer deeper with each recurrent iteration.

\aawarning{Maybe, after each motivational paragraph, include a box environment or something with: ``Ingredient: Blah''. Possible organization: paragraph provides motivation, box title is generic description of technique, and box body is the specific implementation details in our setting? Can also make the boxes referenceable so that in the next section I can say Cts Latent space supervision line incorporates ingredients 1, 2, discrete latent supervision incorporates 1,2,3, etc.}

\aanote{However, we should note somewhere (maybe in discussion), that one of the key advantages of standard linear CoT training is its great versatility (as well as alignment with human thinking). CoT training is easily compatible with the format of (large) language models, which must be able to perform a large number of tasks simultaneously. Standard CoT settings achieve this by simply representing in the reasoning chain in natural human-readable language in the model's original token vocabulary. Moreover, standard CoT training methods produce models with natural human interfaces since humans themselves can only perform deliberate reasoning linearly.}

% above: suggest that latent space should be supervised directly, rather than hack-y autoregressive linear sequential CoT training

% scalability and recurrence

\textbf{\textit{Recurrence \& Input-Adaptive Scaling of Computation Time}.}
Standard autoregressive chain-of-thought methods produce reasoning chains across the length of the autoregressive generation process. A different, more efficient, means of scaling reasoning is across the layer-wise depth of the network. That is, the network performs its reasoning entirely in its latent representation by iteratively performing computation at each layer. To achieve out-of-distribution generalization to larger problems than seen during training, the network architecture must support input-adaptive compute scalability. That is, to solve larger problems, the problem must be able to scale its computation time accordingly. A natural way of achieving this is through recurrent structure---the model learns a recursive computation that is applied iteratively to solve progressively harder problems.

% Implementation: The model architecture consists of a recurrent Transformer module, including some number of Transformer layers each consisting of Attention Followed by a position-wise MLP, which is applied recurrently several times on the given input. We scale the number recurrent iterations so that larger inputs are processed via a larger number of iterations, scaling computation time. [Maybe put this above the algorithmic supervision? Does it come first? Or is this occay.]

\textbf{\textit{Pinning to a Shared Latent Representation via Discretization}.}
One challenge that arises in such recurrent models when they are applied far outside their training distribution to much larger inputs is that their internal vector representations begin to deviate away from the original representation space. Eventually, these ``errors'' accumulate and the embeddings veer far enough away that the model's performance degrades on these large inputs. To address this challenge, we introduce discretization in between recurrent computational blocks as an architectural mechanism to \textit{pin} the representations to a shared space across computational depth.

% Implementation: we give the model a factored embedding space that corresponds to the different factors being supervised, including tokens representing ``\token{\empty}'' for values that are yet to be computed.

\aanote{Can this be visually represented for the continuous-space latent supervision model? Create a plot to this effect}

\textbf{\textit{Learning to Self-Correct}.} In a reasoning task, each reasoning step depends crucially on the prior steps in the reasoning path. If a mistake is made at any stage, all subsequent computation is affected, and the error is often fatal. As the size of the problem and the number of computational steps scale, the likelihood of an error occurring at \textit{some point} in the reasoning process becomes large, limiting the ability to generalize indefinitely to larger and harder problems. To address this challenge, a reasoning model must be able to detect and correct errors as they occur in order to recover when a mistake is made in its previous computation.

% Implementation: with some probability, we randomly corrupt the model's latent state and its ``previous work/computation''. I.e., for a random selection of values that the model computed already, we randomly replace them with a wrong value.

% We observe that our model learns to correct its own mistakes about 50\% of the time, even without explicit supervision on error correction. Motivated by this observation, we carry out additional experiments where we provide explicit supervision to train the model to detect and correct errors in its previous computational steps. [[Describe this process.]] We find that this results in improved error correction capabilities, where the model now corrects nearly 100\% of its errors, boosting the overall full sequence accuracy to nearly 100\%.

\aawarning{In the end, provide complete end-to-end description of the architecture? Include figure.}

% \begin{figure}
%     \centering
%     \includegraphics{figs/experiment_results/ourmethod_stepwise_results/ourmethod_stepwise_results_Blues.pdf}
%     \caption{Robust (easy-to-hard) out-of-distribution Generalization via Input-Adaptive Scaling of Computation Time.}
%     \label{fig:ourmethod_stepwise_results}
% \end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/experiment_results/method_ood_comparison/method_ood_comparison_legendtop.pdf}
%         \caption{Subfigure 1 caption.}
%         \label{fig:subfigure1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/experiment_results/ourmethod_stepwise_results/ourmethod_stepwise_results_Blues.pdf}
%         \caption{Subfigure 2 caption.}
%         \label{fig:subfigure2}
%     \end{subfigure}
%     \caption{A subfigure version}
%     \label{fig:enter-label}
% \end{figure}

\begin{figure}
    \begin{minipage}{0.52\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/experiment_results/method_ood_comparison/method_ood_comparison_legendtop.pdf}
        \captionof{figure}{Out-of-Distribution generalization performance of different methods on the mathematical reasoning task.}
        \label{fig:method_ood_comparison}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.42\textwidth}
            \centering
            \vskip 40pt
            \includegraphics[width=\linewidth]{figs/experiment_results/ourmethod_stepwise_results/ourmethod_stepwise_results_Blues.pdf}
            \captionof{figure}{Robust out-of-distribution generalization via input-adaptive scaling of computation time.}
            \label{fig:ourmethod_stepwise_results}
    \end{minipage}
\end{figure}

\aanote{Rename \methodhighlight{Latent Space Supervision} to \methodhighlight{Latent State Supervision}? Also, remove parentheses from ``(Continuous)''. Maybe use \texttt{textsc} (small caps)? And update text.}
\aanote{Given how strong these results are, we could try to run experiments that target generalization even further beyond $4 \times$ larger. Might also consider extension via fine-tuning trained model by only expanding vocab and embedder, while keeping the rest of the network fixed.}
\aanote{For the second figure: maybe highlight the $N = 32$ line in some way. Maybe via line style, or making it a special color, etc. This gives a visual contrast separating the in distribution regime from out of distribution regime. Also, can maybe indicate the max number of recurrent iterations during training at $T = 10$.}
\aanote{For second figure: could maybe reduce number of lines (i.e., number of node splits) and only include lines in legend. Decrease legend title font size?}

\aanote[inline,nomargin]{Add appendix section for details of training and evaluation. E.g., number of samples, hyperparameter search, teacher-forcing across depth, embedding structure, etc...}

\subsection{Experimental Results, Analysis, \& Discussion}

Combining these different mechanisms together yields an architecture that can robustly generalize far outside the training distribution to much larger inputs. We recall that out-of-distribution generalization on this task requires an ability to generalize in length \textit{and} in computational depth.

\aanote{TODO---add reference to ``ingredient'' boxes once added.}
\aanote{Is the color-coding of method names helpful and aesthetically pleasant? Or should we omit the color-coding (but keep typographic emphasis)?}

\textbf{\textit{A Dramatic Improvement in Out-of-Distribution Generalization.}} \Cref{fig:method_ood_comparison} depicts the out-of-distribution generalization performance of several versions of our method, ablating across the ingredients described above, as well as the aforementioned \methodcolorhighlight{cotsupervisioncolor}{Chain-of-Thought} and \methodcolorhighlight{feedforwardcolor}{End-to-End} baselines. As previously mentioned, we find that the end-to-end models fail to robustly learn the task (with respect to our stringent ``fully solved'' metric) beyond small graph sizes, even in-distribution. The recurrent models slightly outperform the feedforward models. Chain-of-Thought supervision enables a significant improvement, yielding near-perfect performance in-distribution, and a limited degree of out-of-distribution generalization. To assess our proposed ``ingredients'' for robust OOD generalization in Transformers, we evaluate three classes of models incorporating different subsets of those ingredients. We find that this enables a dramatic improvement in OOD generalization, with further improvement the more ingredients are incorporated. When all proposed ingredients are incorporated, the model robustly achieves near-perfect performance across all OOD splits we examined.

\textbf{\textit{The Importance of Pinned Discrete Representations.}} In~\Cref{fig:method_ood_comparison}, \methodcolorhighlight{continuoussupervisioncolor}{Continuous Latent Space Supervision} denotes a recurrent model where the continuous latent states receive step-by-step algorithmic supervision, but the latent states are not discretized in between recurrent block iterations as they are in \methodcolorhighlight{discretesupervisioncolor}{Discrete Latent Space Supervision}. We see that, while this outperforms the chain-of-thought baseline which is limited to linear reasoning paths, its out-of-distribution performance slowly degrades as we test on progressively larger inputs which require increasing recurrent depth and computation time. We attribute this to accumulating noise in the continuous vector representations as we scale test-time compute in order to solve larger problem instances that eventually steer the model away from the semantically-meaningful embedding space that the model understands. In \methodcolorhighlight{discretesupervisioncolor}{Discrete Latent Space Supervision}, the model receives step-by-step algorithmic supervision as with its continuous counterpart, but now we additionally discretize the latent representation, then re-embed using a common embedder that is shared across recurrent iterations. This has the effect of ``pinning'' the latent states to a common, semantically-consistent representation space, allowing the model to scale up computational depth without accumulating noise. We observe that this yields significantly improved OOD generalization.
\aanote{Can this be related, intuitively, to ideas from coding theory? Channel coding, etc.}
\aanote{This resembles the method explored in~\cite{dengImplicitChainThought2023,dengExplicitCoTImplicit2024}, where the continuous hidden states of the model are utilized for reasoning. {TODO--Look at this work in more detail, and see if there is any other relevant work to cite here. Include in discussion/related work.}}

\textbf{\textit{Error-Correction Leads to Greater Robustness in Scaling.}} In our initial experiments, we found that, even without explicitly training the model to correct its errors, the \methodcolorhighlight{discretesupervisioncolor}{Discrete Latent Space Supervision} model is able to correct errors from the previous iteration about 50\% of the time per step. In \methodcolorhighlight{discretesupervisionrecorrectioncolor}{Discrete Latent Space Supervision $\circlearrowleft$}, we introduce explicit supervision for error correction by randomly corrupting the model's latent space with some small probability during training. This boosts the 1-step error correction probability to nearly 100\% and in turn enables robust near-perfect OOD generalization across all OOD splits. Interestingly, we find that error correction requires more layers in the recurrent block in order to succeed. This is intuitive, since it requires additional computational depth from the model per-step to first detect and correct errors from previous steps, before performing the computation for the current step.

\textbf{\textit{Robust Test-time Scaling.}} On many tasks of interest, solving larger problem instances requires scaling computation time accordingly. In order to solve problems larger than those seen during training, we need to scale computation time beyond the training regime. In this work, since the model's reasoning states are latent, we achieve this by scaling the number of recurrent iterations applied to the input. \Cref{fig:ourmethod_stepwise_results} depicts the proportion of input instances that are fully solved with each number of recurrent iterations. Increasing the number of iterations enables solving incrementally larger and harder problem instances. The aforementioned architectural mechanisms are crucial to enabling robust scaling beyond the training regime.
\aanote{Contrast this with prior work on test-time scaling, where it is found that there are hard limits and performance plateaus. E.g.,~\cite{geipingScalingTestTimeCompute2025}: does not really scale beyond the training regime. I.e., scaling compute inside the training range improves performance, but increasing the number of iterations beyond the training regime does not yield improved performance.}

\textbf{\textit{Details, Extensions \& Further Ablations.}} In~\Cref{sec:cot_details,sec:latent_supervision_details,sec:experiments_additional_operations} we provide further discussion and present additional experimental results. Here, we briefly highlight a few aspects of these extensions. Across all methods, we find that hyperparameter choice can be essential. In particular, we find that the choice of positional encoding and model depth is especially important. In the above results, we always report the best model with each method after a hyperparameter search, the details of which are provided in the appendix. Additionally, for the chain-of-thought baselines, we explore multiple schemes for the design of the reasoning chains and present the best results here. We also discuss applying our method to more challenging task setups with multiple arithmetic operations.

% Here, we will focus on a version of the task with a single operation, modular addition, since our focus is on studying out-of-distribution generalization, and traditional methods such as linear chain-of-thought training fail even in this simpler setting. In~\Cref{sec:experiments_additional_operations} we apply our method to a more complex setting with several operations, where the model must learn several operations.

Now that we've demonstrated the effectiveness of the proposed architectural mechanisms for robust OOD generalization, we proceed to carry out a mechanistic interpretability analysis to probe the precise computational circuits learned by each component of our model.


==> preamble.tex <==
% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2025

% % ready for submission
% \usepackage[nonatbib]{neurips_2025}
% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
% %     \usepackage[preprint]{neurips_2025}
% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_2025}
% % to avoid loading the natbib package, add option nonatbib:
% %    \usepackage[nonatbib]{neurips_2025}


\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors
\usepackage{pifont}
\usepackage{fontspec}
\usepackage{stackengine}

\usepackage{color}
% \usepackage[dvipsnames]{xcolor}  % Commented out to prevent option clash with arxiv_preamble.sty

\usepackage{parskip}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{enumitem}

% \usepackage{footnote}
% \makesavenoteenv{tabular} % this allows footnotes inside tabular
% \makesavenoteenv{table}


\usepackage{empheq}

\usepackage{pgfplots}
\pgfplotsset{compat=1.18}

\usepackage{tikz}
\usetikzlibrary{
    shapes.geometric,
    positioning,
    arrows.meta,
    patterns,
    calc
}

% \usepackage{hyperref} % already loaded by pdfcomment below
% \usepackage{color}


\usepackage{setspace}
\usepackage{algorithm2e}
\RestyleAlgo{ruled}
\usepackage[
backend=biber, 
% style=alphabetic, sorting=anyvt,
style=numeric-comp, sorting=none,
maxbibnames=15, url=false, isbn=false, doi=false, natbib=true, backref=true]{biblatex}
\DefineBibliographyStrings{english}{%
  backrefpage = {cited on page},% originally "cited on page"
  backrefpages = {cited on pages},% originally "cited on pages"
}
\AtEveryBibitem{%
  \clearfield{volume}%
  \clearfield{number}
  \clearfield{pages}}
\DeclareFieldFormat{title}{\mkbibquote{#1}}
\addbibresource{references.bib}

% region set up fixme and in-text annotations
\usepackage{pdfcomment}
% put draft in options if, otherwise remove
\usepackage[noinline, margin, index, mode=multiuser, author=]{fixme}
% \usepackage[draft, noinline, margin, index, mode=multiuser, author=]{fixme}
% \usepackage[noinline, margin, mode=multiuser, author=]{fixme}
\usepackage[us]{datetime}
\fxloadlayouts{pdfcnote}

\fxuseenvlayout{colorsig} % plain, signature, color, colorsig
\fxusetargetlayout{changebar} % plain, changebar, color, colorcb

\FXRegisterAuthor{aa}{anaa}{\color{NavyBlue}Awni}
\FXRegisterAuthor{sc}{ansy}{\color{RedViolet}Siyu}
\FXRegisterAuthor{zy}{anzy}{\color{RubineRed}Zhuoran}

\fxusetheme{colorsig}

\fxsetface{inline}{\itshape}
\fxsetface{margin}{\scriptsize\itshape}

% color palete for notes, warning, fatal: color palette (https://coolors.co/palette/f94144-f3722c-f8961e-f9844a-f9c74f-90be6d-43aa8b-4d908e-577590-277da1)
\definecolor{fxnote}{HTML}{43AA8B}
\definecolor{fxwarning}{HTML}{F3722C}
\definecolor{fxfatal}{HTML}{F94144}

% hyperref set up
\hypersetup{%
    %draft, % = no hyperlinking at all (useful in b/w printouts)
    colorlinks=true, linktocpage=true, pdfstartpage=3, pdfstartview=FitV,%
    % uncomment the following line if you want to have black links (e.g., for printing)
    %colorlinks=false, linktocpage=false, pdfstartpage=3, pdfstartview=FitV, pdfborder={0 0 0},%
    breaklinks=true, pdfpagemode=UseNone, pageanchor=true, pdfpagemode=UseOutlines,%
    plainpages=false, bookmarksnumbered, bookmarksopen=true, bookmarksopenlevel=1,%
    hypertexnames=true, pdfhighlight=/O,%nesting=true,%frenchlinks,%
    % urlcolor=BrickRed, linkcolor=RoyalBlue, citecolor=teal, %pagecolor=RoyalBlue,%
    urlcolor=BrickRed, linkcolor=magenta, citecolor=magenta, %pagecolor=RoyalBlue,%
    %urlcolor=Black, linkcolor=Black, citecolor=Black, %pagecolor=Black,%
    % pdftitle={\myTitle},%
    % pdfauthor={\textcopyright\ \myName, \myUni, \myFaculty},%
    % pdfauthor={\myName},%
    pdfsubject={},%
    pdfkeywords={},%
}


% color-coding
\newcommand{\inprog}[1]{{\color{Gray} #1}}
\newcommand{\edit}[1]{{\color{BrickRed} #1}}
\newcommand{\add}[1]{{\color{Emerald} #1}}
\newcommand{\trim}[1]{{\color{red}}}
\newcommand{\delete}[1]{{\color{red} \sout{#1}}}
\newcommand{\remove}[1]{{\color{red} #1}}
\newcommand{\replace}[2]{\delete{#1} \add{#2}}
% endregion

% my packages / macros /etc
\usepackage{mymathstyle}
\usepackage{paper_commands}
% \usepackage{boxes}
\usepackage{mechanism_boxes}

% set default bullet for itemize
\setlist[itemize]{label=$\circ$}

% emphasis
% \renewcommand{\emph}[1]{{\color{magenta} \textit{#1}}}


